Cross-Dataset Gaze Estimation by Evidential Inter-intra Fusion

Achieving accurate and reliable gaze predictions in complex and diverse environments remains challenging. Fortunately, it is straightforward to access diverse gaze datasets in real-world applications. We discover that training these datasets jointly can significantly improve the generalization of gaze estimation, which is overlooked in previous works. However, due to the inherent distribution shift across different datasets, simply mixing multiple dataset decreases the performance in the original domain despite gaining better generalization abilities. To address the problem of ``cross-dataset gaze estimation'', we propose a novel Evidential Inter-intra Fusion EIF framework, for training a cross-dataset model that performs well across all source and unseen domains. Specifically, we build independent single-dataset branches for various datasets where the data space is partitioned into overlapping subspaces within each dataset for local regression, and further create a cross-dataset branch to integrate the generalizable features from single-dataset branches. Furthermore, evidential regressors based on the Normal and Inverse-Gamma (NIG) distribution are designed to additionally provide uncertainty estimation apart from predicting gaze. Building upon this foundation, our proposed framework achieves both intra-evidential fusion among multiple local regressors within each dataset and inter-evidential fusion among multiple branches by Mixture \textbfof Normal Inverse-Gamma (MoNIG distribution. Experiments demonstrate that our method consistently achieves notable improvements in both source domains and unseen domains.

==> sec/4_exp_origin.tex <==
\section{Experiment}
\subsection{Cross-dataset Setting}
The experiments utilize four widely used gaze estimation datasets, EyeDiap~\cite{funes2014eyediap}, MPIIFaceGaze~\cite{zhang2017mpiigaze}, Gaze360~\cite{kellnhofer2019gaze360}, and ETH-XGaze~\cite{zhang2020eth}. We pre-process the data following the technique in~\cite{cheng2021appearance}. To facilitate comparisons, we reference the setup of cross-domain scenarios~\cite{xu2023learning, Cai_2023_CVPR} in our cross-dataset setting, \textit{i.e.,} we choose ETH-XGaze and Gaze360, known for their wider gaze distributions and larger data volumes, as the source domains, and MPIIGaze and EyeDiap as the target datasets. Detailed information about the datasets can be found in the Supplementary Material.

% \textbf{ETH-Gaze (Source Domain):} This dataset was captured in a laboratory environment using high-resolution cameras and consists of 756,000 training images from 80 subjects. Since the ETH-Gaze dataset does not include gaze target annotations for the test set, we redefine the dataset splits following the approach in \cite{cheng2021appearance}. Specifically, we split the original training set into two subsets to use as training and testing sets, as done in previous studies \cite{cheng2023dvgaze}. The gaze ranges are ±120° yaw and ±70° pitch.

% \textbf{Gaze360 (Source Domain):} This dataset is collected in both indoor and outdoor environments using a 360-degree camera. It includes 84,000 training images from 54 subjects and 16,000 testing images from 15 subjects, with gaze ranges of ±140° yaw and -50° pitch.

% \textbf{MPIIFaceGaze (Target Domain):} This dataset is captured during natural laptop use, utilizing the laptop camera for image capture. It comprises 45,000 images from 15 users, with gaze ranges of ±20° yaw and ±20° pitch.

% \textbf{EyeDiap (Target Domain):} This dataset is collected in a laboratory setting, where participants are instructed to gaze at two types of visual targets: screen targets and a 3D floating ball. It contains a total of 16,000 images from 16 users, with gaze ranges of ±25° yaw and ±20° pitch.

\subsection{Implementation Details}
We use ResNet-18 backbone following previous studies \cite{cheng2022puregaze, Cai_2023_CVPR, bao2024feature}. All images are resized to 224 × 224, and we use the Adam optimizer with a learning rate of \(10^{-4}\).
In Stage 1, we train on each source domain dataset for 100k batches. Specifically, for the Gaze360 single-dataset branch, we use the ETH-Gaze’s backbone for pre-training, similar to previous work~\cite{cheng2022gaze}.
 In stage 2, we perform joint training for only 5k batches using all source domain datasets. Considering the discrepancy in the quantity of data among source domain datasets, during the joint training in stage 2, instead of directly mixing multiple datasets for sampling, we adopt a balanced mixing approach, where the datasets with fewer samples are oversampling to balance the data across all source domain datasets.
By default, we set the number of local regressors \( G \) to 8, the overlap coefficient \( \alpha \) to 2.0, the evidence learning regularization loss \( \lambda \) to 0.01, the dataset split ratio in stages 1 and 2 to 4:1, and the starting MFF layer \( K \) in the cross-dataset branch to 3.

\begin{table*}[t]
\centering
\small
\caption{Comparison of gaze estimation performance in terms of angle error (°) in domain generalization setting. The best, second best, and third best results are denoted as \BEST{red}, \SBEST{blue}, and \TBEST{green}, respectively. † indicates the reproduced cross-domain gaze estimation results.}
\label{tab:cross_dataset_training}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}ccccccccc@{}}
\toprule
\multicolumn{3}{c}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Source Domain}} & \multicolumn{2}{c}{\textbf{Target Domain}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
\textbf{Type} & \textbf{Name} & \textbf{Train Data} & \textbf{ETH} & \textbf{G360} & \textbf{EyeDiap} & \textbf{MPII} & \textbf{Target} & \textbf{All} \\
\midrule
\multirow{2}{*}{\shortstack{Single-dataset\\Baseline}} 
& Baseline & ETH & \SBEST{4.55} & 20.70 & 10.70 & 8.46 & 9.58 & 11.10 \\
& Baseline & G360 & 16.90 & 11.21 & 10.90 & 7.23 & 9.07 & 11.56 \\
\midrule
\multirow{2}{*}{\shortstack{Cross-dataset\\Baseline}} 
& Simple Mixing & G360 & \TBEST{4.68} & 11.42 & \SBEST{6.42} & 6.95 & 6.69 & \TBEST{7.37} \\
& Balanced Mixing & ETH+G360 & 4.90 & \SBEST{10.76} & \BEST{6.40} & \SBEST{6.50} & \SBEST{6.45} & \SBEST{7.14} \\
\midrule
\multirow{2}{*}{\shortstack{Multi-source\\Domain Generalization}}
& GMDG\cite{tan2024rethinking} & ETH+G360 & 4.76 & \TBEST{10.95} & 7.12 & 7.07 & 7.10 & 7.48 \\
& BNE\cite{segu2023batch} & ETH+G360 & 5.44 & 11.06 & 6.73 & \TBEST{6.51} & \TBEST{6.62} & 7.44 \\
\midrule
\multirow{4}{*}{\shortstack{Cross-domain\\Gaze Estimation}} 
& PureGaze\cite{cheng2022puregaze} & ETH & 4.77† & 21.67† & 7.08 & 7.48 & 7.28 & 10.25 \\
& PureGaze\cite{cheng2022puregaze} & G360 & 17.11† & 11.21† & 9.28 & 9.32 & 9.30 & 11.73 \\
& AGG~\cite{bao2024feature} & ETH & 5.56 & - & 7.07 & 7.10 & 7.09 & - \\
& AGG~\cite{bao2024feature} & G360 & - & 13.03 & 7.93 & 7.87 & 7.90 & - \\
\midrule
\multirow{1}{*}{Our Method} 
& EIF & ETH+G360 & \BEST{4.42} & \BEST{10.46} & \TBEST{6.45} & \BEST{6.01} & \BEST{6.23} & \BEST{6.84} \\
\bottomrule
\end{tabular*}
\end{table*}

\subsection{Domain Generalization Results}
We trained our method on the source domains (ETH-Gaze and Gaze360) and compared it with four types of methods:

\textbf{Single-dataset Baseline:} These methods are trained on a single source domain using the standard L1 loss function for gaze estimation, while other network settings remain consistent with those of our proposed method.

\textbf{Cross-dataset Baseline:} These methods are trained on ETH-Gaze and Gaze360 using two different mixing strategies: \textbf{Simple Mixing}, where the datasets are directly concatenated, and \textbf{Balanced Mixing}, which, similar to our Stage 2 method, uses balanced sampling. The network and training settings are kept identical to those in the single-dataset baseline.

\textbf{Multi-source Domain Generalization:} These methods implement solutions for Multi-source Domain Generalization, which combines multiple source domains to improve performance in the target domain, making them relevant to our scenario. We implement two representative methods: GMDG~\cite{tan2024rethinking}, a domain alignment approach for regression tasks, and BNE~\cite{segu2023batch}, which shares convolutional layers while maintaining independent batch normalization across domains, similar to cross-dataset training in autonomous driving~\cite{wang2022cross}. The other training settings are consistent with those in the balanced mixing cross-dataset baseline.

\textbf{Cross-domain Gaze Estimation:} These methods are state-of-the-art gaze estimation domain generalization approaches. They are trained on a single source domain (ETH-Gaze or Gaze360) using carefully designed algorithms for domain generalization.

From Table \ref{tab:cross_dataset_training}, it can be observed that the cross-dataset baseline  achieves comparable performance with the carefully designed SOTA single-domain generalization methods on the target dataset. However, there is a slight error increase in the source domains. Multi-source Domain Generalization fails to bring improvements and may even slightly degrade performance. In contrast, our proposed method EIF reduces gaze errors in both the source domains (ETH-Gaze by 0.48° and Gaze360 by 0.30°) and the target domains (by 0.22°) compared to the best cross-dataset baseline(balanced mixing), ultimately surpassing the best  cross-domain generalization method AGG~\cite{bao2024feature} (ETH-Gaze) by a large improvement (ETH-Gaze by 1.14°, target domains by 0.86°).

\subsection{Domain Adaptation Results} %with target Domain Data}
Our previous experiments demonstrate the effectiveness of our method both in the source domain and in generalizing to target domains. To further validate the efficacy of our EIF framework, as done in previous domain generalization works~\cite{cheng2022puregaze, bao2024feature}, we conduct domain adaptation experiments. 

Similar with previous domain adaptation setting, we fine-tune the model using 100 images from the target domain over 100 batches. For our EIF, we use these data to constrain the evidence loss (Equation \ref{equation:evidence_regression_learning}), both for all branches and their joint output after inter-fusion. To mitigate randomness resulting from the random sampling of the training set, we repeat the experiment 5 times and report the average results. 

% As demonstrated in Table \ref{table: domain adaption}, our method significantly outperforms previous state-of-the-art (SOTA) approaches after being fine-tuned with a limited number of samples from target domains. Notably, our approach achieves a reduction in angular error of 0.68° on MPIIFace and 0.20° on EyeDiap (\textit{i.e.}, an average improvement of 8.64\% in target domains) compared with the previous best method.
As shown in Table \ref{table: domain adaption}, our EIF framework significantly improves domain adaptation performance, reducing the error by 0.62° compared to the best cross-domain method, PureGaze (ETH-Gaze).

\begin{table}[h]
\centering
\tabcolsep=1.5mm
\caption{Comparison with SOTA methods in domain adaptation on 100 labeled samples. Results are shown in angle error (°).}
\label{table: domain adaption}
\begin{tabular} {lccc}
%\hline
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Target Dataset} & \multirow{2}{*}{Avg}\\
\cmidrule(lr){2-3}
& MPII & EyeDiap \\
%\hline
\midrule
PureGaze (ETH-Gaze)~\cite{xu2023learning} & 4.76 & 5.43 & 5.10\\
PureGaze (Gaze360)~\cite{xu2023learning} & 5.34 & 5.66 & 5.50\\
AGG (ETH-Gaze)~\cite{bao2023pcfgaze} & 4.74 & 5.88 & 5.31\\
AGG (Gaze360)~\cite{bao2023pcfgaze} & 5.41 & 6.39 & 5.90 \\
\midrule
EIF (ETH-Gaze+Gaze360) & \textbf{3.91} & \textbf{5.04} & \textbf{4.48}\\
%\hline
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

\subsection{Ablation Study}
Since our model consists of two stages, each serving a clear purpose: the first stage single-dataset training involves training a well-performing evidence learning regression branch for each dataset, while the second stage cross-dataset joint training entails fusing these branches based on evidence learning to achieve a model with superior generalization capability. Hence, for clarity, we conduct ablation experiments in two parts accordingly.%, mirroring the stages.

\textbf{Single-dataset training:} To train a well-performing single-dataset evidence learning regression branch, we primarily include two components: firstly, introducing evidential regression learning, and secondly, incorporating multiple local regressors corresponding to specific data subspaces and utilizing intra-evidential fusion to aggregate them.
\begin{table}[t]
\centering
\caption{Ablation study of the single-dataset training  on the Gaze360 Dataset.}
\scalebox{0.9}{
\begin{tabular}{ccc|c}
\hline
\begin{tabular}[c]{@{}c@{}}L1 \\ Regression\end{tabular} & \begin{tabular}[c]{@{}c@{}}Evidential \\ Regression\end{tabular} & \begin{tabular}[c]{@{}c@{}}Intra-Evidential \\ Fusion\end{tabular} &  Angle Error(°)  \\ \hline
 $\checkmark$  & &  &  4.55  \\
 & $\checkmark$  &  &  4.59  \\
 & $\checkmark$  &$\checkmark$   & \textbf{4.35} \\ \hline
\end{tabular}}
\label{table: ablation_study_single_dataset}
\end{table}
As shown in Table~\ref{table: ablation_study_single_dataset}, we conduct ablation studies to evaluate the effectiveness of each components mentioned above: 1) Evidence regression: To estimate uncertainty, evidential regression introduces more complex distributions to model the regression, resulting in a slight error increase of 0.05°. However, this provides the foundation for our inter-intra evidence fusion; 2) Intra-evidential fusion: Compared to using only evidential regression in gaze estimation, the approach with the intra-evidential fusion strategy significantly reduces the angle error by 0.24°, surpassing the baseline method without evidence regression by 0.20°.
% \textbf{Single-Dataset training.} To train a well-performing single dataset evidence learning regression branch, we follow these steps:(1) We first introduce evidence regression learning.(2) Then, we further partition the dataset into multiple gaze groups and assign a local regressor to each group. We utilize itra-evidential fusion module to aggregate their predictions.(3) When partitioning the dataset, we employ a dense overlap strategy among gaze groups. This strategy ensures that data within overlapping regions contribute to training multiple regressors, thereby enhancing the robustness of the model. 
% \begin{table}[ht]
% \centering
% \caption{Single-Dataset Training Ablation Study on the ETH-Gaze Dataset.}
% \scalebox{0.9}{
% \begin{tabular}{ccc|c}
% \hline
% \begin{tabular}[c]{@{}c@{}}Evidential \\ Regression\end{tabular} & \begin{tabular}[c]{@{}c@{}}Intra-Evidential \\ Fusion\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gaze Group \\ Overlap\end{tabular}& Angle Error(°)  \\ \hline
%   &  &  & 5.02  \\
%  $\checkmark$  &  &  & 5.07  \\
%  $\checkmark$  &$\checkmark$  &  &  \\
%  $\checkmark$  &$\checkmark$  &$\checkmark$  & \textbf{4.88} \\ \hline
% \end{tabular}}
% \label{table: ablation_study_single_dataset}
% \end{table}
% Now, as shown in Table \ref{table: ablation_study_single_dataset}, We conduct ablation studies to evaluate the effectiveness of each step mentioned above. \textbf{Evidence Regression}: To estimate uncertainty, evidential regression introduces more complex distributions to model the regression, resulting in a slight decrease of 0.05°. However, this provides the foundation for our inter-intra evidence fusion. \textbf{Intra-Evidential Fusion}: Compared to using only evidential regression in gaze estimation, the approach with the intra-evidential fusion strategy significantly reduces the angle error by &°, surpassing the baseline method without evidence regression by &°. \textbf{Gaze Group Overlap}: This gaze group partitioning strategy further reduces the angle error by &°.

\begin{table}[t]
\centering
\caption{Ablation study for cross-dataset joint training. This study showcases the average angle errors (°) of the models trained on multiple source domains (ETH-Gaze+Gaze360) across the source domain test sets (ETH-Gaze and Gaze360) and the target domains (MPIIFaceGaze and EyeDiap).}
\scalebox{0.85}{
\begin{tabular}{ccc|cc}
\hline
\begin{tabular}[c]{@{}c@{}}
Average \\ Fusion\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inter-Evidential \\ Fusion\end{tabular} & \begin{tabular}[c]{@{}c@{}}Cross-Dataset \\ Branch \end{tabular} &  Source & target  \\ \hline
 $\checkmark$  & &  &  11.32  & 6.86\\
 & $\checkmark$  &  &  7.47  & 6.67 \\
 & $\checkmark$  &$\checkmark$   & \textbf{7.44}  & \textbf{6.23} \\ \hline
\end{tabular}}
\label{table: ablation_cross_dataset_jointly}
\end{table}

\textbf{Cross-dataset joint training:} To jointly train multiple single-dataset branches, we first adopt the inter-evidential fusion module to aggregate predictions from multiple branches. Additionally, we further designed a cross-dataset branch to integrate features from each branch.
As shown in Table~\ref{table: ablation_cross_dataset_jointly}, we conduct ablation studies to evaluate the effectiveness of each module mentioned above. All the single-dataset branches used in this experiment are based on the intra-evidential fusion approach. The experimental result shows that inter-evidential fusion approach exhibits a significant reduction in errors compared to directly averaging prediction of each branch after stage 1 (Average Fusion), with reductions of 3.85° and 0.19° in the source and target domains, respectively. These results match the preliminary experiment and clearly verify our intuition that aggregating predictions from multiple source domains with diverse distribution is beneficial for generalization even when employing a simple average fusion strategy. However, this simply fusion approach may compromise performance in the source domain. In contrast, our inter-fusion method not only significantly boosts performance in the source domain but also further amplifies it in the target domain. Moreover, our cross-dataset branch further enhances the performance of the inter-evidential fusion, with reductions of 0.03° and 0.44° in the source and target domains, respectively. This result highly suggests that our designed cross-dataset branch aggregates features from each source domain branch and thus can better fuse a wide range of distributions for generalization to target domains.


\subsection{Parameter Sensitivity Analysis}
In our experiments, we consider two critical hyperparameters: the number of local regressors \(G\) in single-dataset training and the MFF starting layer \(K\) in cross-dataset joint training. We separately conduct experiments to analyze the impact of these hyperparameters.

\textbf{Effects of the number of local regressors in single-dataset training:} As shown in Table \ref{table: G_analysis_results}, we can observe that within a certain range, adjusting the \( G \) has a relatively stable impact on the performance. Specifically, setting the number of local regressors to 8 achieves the best performance.
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table}[t]
\centering
\caption{Parameter analysis in single-dataset training on ETH-Gaze dataset. }
\label{table: G_analysis_results}
\begin{tabularx}{0.8\linewidth}{CCC}
%\hline
\toprule
Parameter & Value & Angle Error (°) \\
%\hline
\midrule
 & 4 & 4.45 \\
 $G$ & 8 & 4.35 \\
 & 32 & - \\
%\hline
\bottomrule
\end{tabularx}
\end{table}

\textbf{Effects of the layer $K$ in cross-dataset joint training:} As shown in Table \ref{table: K_analysis_results}, we can see that within a certain range, adjusting the \( K \) also has a relatively stable impact on the performance. In our experiment, setting \( K \) to 3 achieves the best performance.

\begin{table}[h]
\centering
\caption{Parameter analysis in cross-dataset training. Results are shown in angle error (°).}
\label{table: K_analysis_results}
\begin{tabular}{ccccccc}
%\hline
\toprule
\multirow{2}{*}{Param} & \multirow{2}{*}{Value} & \multicolumn{5}{c}{Dataset} \\
\cmidrule(lr){3-7}
& & ETH & G360 & Diap & MPII & Avg\\
%\hline
\midrule
 & 2 & 4.40 & 10.45 & 6.45 & 6.2 & 6.88\\
 $K$ & 3 & 4.42 & 10.46 & 6.45 & 6.01 & \textbf{6.84} \\
 & 4 & 4.43 & 10.47 & 6.49 & 6.14 & 6.88 \\
%\hline
\bottomrule
\end{tabular}
\end{table}

% In our experiments, we considered two critical hyperparameters: the number of local regressors \(G \) and the MFF starting layer \( K \) in the cross-dataset branch. We analyzed the impact of hyperparameter settings in this experiment. As shown in Table \ref{table:parameter_analysis_results}, we observed that within a certain range, adjusting the hyperparameters had a relatively stable impact on the performance. Specifically, setting the number of local regressors to 8 and the starting layer \( K \) to 3 achieved the best overall performance.


% \begin{table}[h]
% \centering
% \caption{Parameter analysis in cross-dataset training. Results are shown in angle error(°).}
% \label{table:parameter_analysis_results}
% \begin{tabular}{ccccccc}
% %\hline
% \toprule
% \multirow{2}{*}{Param} & \multirow{2}{*}{Value} & \multicolumn{5}{c}{Dataset} \\
% \cmidrule(lr){3-7}
% & & Gaze360 & ETH & MPII & EyeDiap & Avg\\
% %\hline
% \midrule
%  & 4 & 11.48 & 4.97 & 6.78 & 7.90 & 7.78 \\
% $G$  & 8 & 11.33 & 4.95 & 6.41 & 6.90 & \textbf{7.40}\\
%  & 16 & 11.33 & 4.96 & 7.05 & 7.62 & 7.74 \\
% %\hline
% \midrule
%  & 2 & 11.39 & 4.96 & 6.20 & 7.22 & 7.44\\
%  $K$ & 3 & 11.33 & 4.95 & 6.41 & 6.90 & \textbf{7.40} \\
%  & 4 & 11.36 & 4.95 & 6.36 & 7.21 & 7.47 \\
% %\hline
% \bottomrule
% \end{tabular}
% \end{table}


\subsection{Evidence Analysis}
Evidential learning is crucial to our framework; we use it to achieve an inter-intra fusion, and the final evidential regression output can also provide uncertainty estimations for robust predictions. Therefore, in this section, we offer a visual analysis of the fusion process and uncertainty predictions to validate the effectiveness of evidential learning in gaze estimation.


\textbf{Inter-intra fusion visual analysis:} 
Based on Equation \ref{equation:evidence_regression_learning}, among the four output values of the evidential regression, \(\delta\) represents the predicted gaze. Furthermore, according to Equation \ref{equation:MoNIG}, during the evidential fusion process, normalized \(\gamma\) is employed as weights to aggregate \(\delta\) accordingly. Hence, to further delve into our inter-intra evidential fusion module, we compute the mean normalized \(\delta\) values spanning multiple local regressors or branches. 

As depicted in Fig.~\ref{image:inter-intra_visualize}(a), the visualization showcases the output on the yaw values of the test set corresponding to the single-dataset branch in ETH-Gaze. It is observable that the diagonal region possesses the highest values, indicating our intra-fusion module enables samples within each gaze group to find their corresponding local regressors effectively. Moreover, it is noted that the weights are not solely concentrated on a single diagonal but are diffused around the diagonal line. This distribution is attributed to our adoption of a density overlap strategy for gaze group segmentation (Equation~\ref{eq:gaze_group_interval}), which allocates multiple experts to one sample in overlapping areas, thereby enhancing robustness. Conversely, due to the lack of overlap in the boundary gaze group areas (0 and 7), the weights are relatively more focused compared to other regions. 

As shown in Fig.~\ref{image:inter-intra_visualize}(b), the experiment is conducted on the complete EIF structure. It demonstrates that all source domain test sets have the highest weights on their respective single-dataset branches. On the other hand, in the target domains, the weights are distributed evenly across various branches.
% Notably, EyeDiap has the highest weight on the cross-dataset branch, while MPIIFaceGaze shows the highest weight on the ETH-Gaze branch. The possible reason is that the single-dataset branch learned on the ETH-Gaze dataset demonstrates a strong generalization capability on MPIIFaceGaze. Previous domain generalization methods in Table~\ref{tab:cross_dataset_training} have also shown that models trained on ETH-Gaze perform well on MPIIFaceGaze, which is consistent with this observation and verifies the effectiveness of our evidential learning fusion strategy.
\begin{figure}
 \centering
 \includegraphics[width=8.5cm]{picture/nus_heatmap.png}
  \caption{Visualizing Weights During Inter-Intra Fusion.}
  \label{image:inter-intra_visualize}
\end{figure}

% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.36\linewidth}
%   \includegraphics[width=\linewidth]{itra_evidential_heatmapETH-Gaze.png}
%   \caption{(a)The average weights for each local regressor during the intra-evidential fusion across different gaze groups.}
%   \label{fig:image1}
% \end{subfigure}
% \quad % Space between images
% \begin{subfigure}{0.58\linewidth}
%   \includegraphics[width=\linewidth]{inter_evidence.png}
%   \caption{(b)The average weights assigned to each single-dataset branch during the inter-evidential fusion across different datasets.}
%   \label{fig:image2}
% \end{subfigure}
% \caption{Visualizing Weights During Inter-Intra Fusion.}
% \label{fig:inter-intra_visualize}
% \end{figure}

\textbf{Uncertainty Estimation Analysis:}
% To analyze the relationship between uncertainty and error, we computed the Pearson correlation coefficient among sample data uncertainty, model uncertainty, and error for our EIF architecture tested across four datasets. Here, the sample uncertainty is calculated as the average of its values for yaw and pitch predictions.
Our model can simultaneously provide epistemic uncertainty and aleatoric uncertainty. Epistemic uncertainty reflects the model's uncertainty about the underlying structure of the data. It arises from the model's lack of knowledge or exposure to certain regions of the input space during training. To avoid the influence of label ranges, we restrict the input gaze to the frontal region (±20°) when computing statistics on epistemic uncertainty. As shown in Fig.~\ref{image:epi_uncer}, the epistemic uncertainty of the target EyeDiap dataset is relatively large in the final output of our EIF structure, while that of the source domains and MPIIFaceGaze is smaller. The smaller uncertainty in MPIIFaceGaze may be due to its similarity to a subset of the source domain datasets.
\begin{figure}
 \centering
 \includegraphics[width=7cm]{picture/Epistemic_uncertainty.png}
  \caption{The epistemic uncertainty of the dataset.}
  \label{image:epi_uncer}
\end{figure}
% \begin{table}[h]
% \centering
% \caption{The epistemic uncertainty of the dataset.}
% \label{table:epi_uncer}
% \begin{tabularx}{0.7\linewidth}{lC}
% %\hline
% \toprule
% Dataset & Epistemic Uncertainty \\
% %\hline
% \midrule
% ETH-Gaze & 2.22e-4 \\
% Gaze360 & 2.87e-4 \\
% MPIIFaceGaze & 1.52e-4 \\
% EyeDiap & 3.29e-4 \\
% %\hline
% \bottomrule
% \end{tabularx}
% \end{table}

The aleatoric uncertainty of the data involves the inherent uncertainty of the data itself, which cannot be eliminated even with a sufficiently large dataset. This uncertainty arises from factors such as low image quality, including reasons like image blur and occlusion of the eyes in our task.
\begin{figure}
 \centering
 \includegraphics[width=7cm]{picture/data_uncertaintyvis.png}
  \caption{The aleatoric uncertainty of two source datasets}
  \label{image:data_uncertainty_visulization}
\end{figure}
As depicted in Fig.~\ref{image:data_uncertainty_visulization}, we showcase the aleatoric uncertainty output of our EIF in the source domain test sets, where ETH-Gaze is collected on a per-user basis, and Gaze360 is collected on a per-scene basis. Therefore, we respectively output the maximum and minimum values of the estimated aleatoric uncertainty for each subject or scene on ETH-Gaze and Gaze360. It can be observed that the aleatoric uncertainty output by our model effectively reflects the data quality in the source domain. More visualization results can be found in the appendix.

\subsection{Computational Cost}
%\textbf{Training Time.} 
Despite encompassing multiple branches, thanks to our two-stage learning strategy, our model can be trained swiftly to adapt to new scenarios. Once we have multiple trained single-dataset branches, our model requires only a minimal number of epochs in stage 2 to rapidly adjust to changes in the dataset, such as additions or deletions. Specifically, in our experiments, the training of stage 2 takes only 40 minutes on two NVIDIA TITAN XP GPU, whereas the baseline needs to start from scratch and mixing multiple datasets, which requires 5 hours for training.

